A Differentiable Recurrent Surface for Asynchronous Event-Based Data

Dynamic Vision Sensors (DVSs) asynchronously stream events in correspondence of pixels subject to brightness changes. Differently from classic vision devices, they produce a sparse representation of the scene. Therefore, to apply standard computer vision algorithms, events need to be integrated into a frame or event-surface. This is usually attained through hand-crafted grids that reconstruct the frame using ad-hoc heuristics. In this paper, we propose Matrix-LSTM, a grid of Long Short-Term Memory (LSTM) cells that efficiently process events and learn end-to-end task-dependent event-surfaces. Compared to existing reconstruction approaches, our learned event-surface shows good flexibility and expressiveness on optical flow estimation on the MVSEC benchmark and it improves the state-of-the-art of event-based object classification on the N-Cars dataset.

==> data/plot_kevent.tex <==
\begin{figure}[th]
\centering
\begin{tabular}{c}
\resizebox{0.8\columnwidth} {!} {
  \begin{tikzpicture}
  \begin{axis}[
      enlargelimits=false,
  axis y line=right,
  axis x line=none,
  yticklabel pos=right,
      legend pos=north east,
      ylabel={K events/s},
      xlabel={batch size},
       xmin=1, xmax=256,
       ymin=0, ymax=6000,
       symbolic x coords={1,2,8,16,32,64,128,256},
      xtick={1,2,8,16,32,64,128,256},
      ytick={1000,2000,3000,4000,5000,6000},
      ymajorgrids=true,
      grid style=dashed,
  ]
  \addplot[
      color=MaterialBlue700,
      mark=oplus*]
  table[x index=0,y index=1,col sep=comma]
  {data/kevents.txt};
  \legend{event rate}
  \end{axis}
  \begin{axis}[
      enlargelimits=false,
      %title={Intersection over Union with varying $\mu_1$, $\mu_2$, $\mu_3$},
      ylabel={mean time(ms)},
      legend pos=north west,
      xlabel={batch size},
       xmin=1, xmax=256,
       ymin=0, ymax=12,
       symbolic x coords={1,2,8,16,32,64,128,256},
      xtick={1,2,8,16,32,64,128,256},
      ytick={0,2,4,6,8,10,12},
      ymajorgrids=true,
      grid style=dashed,
  ]
  \addplot[
      color=MaterialRed700,
      mark=oplus*]
  table[x index=0,y index=1,col sep=comma]
  {data/timing.txt};
  \legend{timing}
  \end{axis}
  \end{tikzpicture}
}
\end{tabular}
\caption{Number of processed events per second and timing }
\label{fig:kevents}
\end{figure}



==> data/plot_timing.tex <==
\begin{figure}[th]
\begin{tabular}{c}
\centering
\resizebox {0.95\columnwidth} {!} {
  \begin{tikzpicture}
  \begin{axis}[
      enlargelimits=false,
      %title={Intersection over Union with varying $\mu_1$, $\mu_2$, $\mu_3$},
      ylabel={batch size},
      xlabel={mean time(ms)},
       xmin=1, xmax=256,
       ymin=0, ymax=12,
       symbolic x coords={1,2,8,16,32,64,128,256},
      xtick={1,2,8,16,32,64,128,256},
      ytick={0,2,4,6,8,10,12},
      legend pos=south east,
      ymajorgrids=true,
      grid style=dashed,
  ]
  \addplot[
      color=MaterialRed700,
      mark=oplus*]
  table[x index=0,y index=1,col sep=comma]
  {data/timing.txt};
  \legend{timing, event rate}
  \end{axis}
  
  \end{tikzpicture}
}
\end{tabular}
\caption{Timings of Matrix-LSTM}
\label{fig:timing}
\end{figure}


